Kubernetes Autoscaling: YoYo Attack Vulnerability and Mitigation

In recent years, we have witnessed a new kind of DDoS attack, the burst attack(Chai, 2013; Dahan, 2018), where the attacker launches periodic bursts of traffic overload on online targets. Recent work presents a new kind of Burst attack, the YoYo attack (Bremler-Barr et al., 2017) that operates against the auto-scaling mechanism of VMs in the cloud. The periodic bursts of traffic loads cause the auto-scaling mechanism to oscillate between scale-up and scale-down phases. The auto-scaling mechanism translates the flat DDoS attacks into Economic Denial of Sustainability attacks (EDoS), where the victim suffers from economic damage accrued by paying for extra resources required to process the traffic generated by the attacker. However, it was shown that YoYo attack also causes significant performance degradation since it takes time to scale-up VMs. In this research, we analyze the resilience of Kubernetes auto-scaling against YoYo attacks. As containerized cloud applications using Kubernetes gain popularity and replace VM-based architecture in recent years. We present experimental results on Google Cloud Platform, showing that even though the scale-up time of containers is much lower than VM, Kubernetes is still vulnerable to the YoYo attack since VMs are still involved. Finally, we evaluate ML models that can accurately detect YoYo attack on a Kubernetes cluster.

==> abstract2.tex <==
In recent years, we have witnessed a new kind of DDoS attack, \anat{ the burst attack \cite{ } }, where the attacker launches periodic bursts of traffic overload on online targets.

\anat{ A variant of the attack }, the YoYo attack,  operates against the auto-scaling mechanism of VMs in the cloud. The auto-scaling mechanism translates the flat DDoS attacks into Economic Denial of Sustainability attacks (EDoS), where the victim suffers from economic damage accrued by paying for extra resources required to process the traffic generated by the attacker. It is a common approach that Auto-scaling mechanism is an important line of defence against DDoS in the cloud. This approach is suggested by an official cloud provider's documentation,  \cite{amazonDDoSwhitepapers} to protect applications availability when there is an unexpected increase in the request volume. Thus, major cloud vendors offer the  auto-scaling technology as a defence in conjunction with an expensive web application firewall (WAF) service. Bursts of traffic causes significant performance degradation in addition to economic damage. The periodic bursts of traffic loads cause the auto-scaling mechanism to oscillate between scale-up and scale-down phases.  As containerized cloud applications gain popularity and replace VM-based architecture, it is important to understand how Kubernetes handles YoYo attacks. In this paper, we analyze the resilience of Kubernetes auto-scaling against YoYo attacks. We model the underlying auto-scaling mechanism and show that it is still very vulnerable to YoYo attacks, because VMs are still involved in this mechanism. Given that, we propose a novel approach to detect a YoYo attack on a Kubernetes cluster based on machine learning methodology.  We demonstrate the YoYo attack and its mitigation on a Google Kubernetes Engine cluster. 

\ignore{In recent years, we have witnessed a new kind of DDoS attack, where the attacker launches periodic bursts of traffic overload on online targets. Known as the YoYo attack, this attack operates against the auto-scaling mechanism of VMs in the cloud. The auto-scaling mechanism translates the flat DDoS attacks into Economic Denial of Sustainability attacks (EDoS), where the victim suffers from economic damage accrued by paying for extra resources required to process the traffic generated by the attacker. Bursts of traffic causes significant performance degradation in addition to economic damage. The periodic bursts of traffic loads cause the auto-scaling mechanism to oscillate between scale-up and scale-down phases.  As containerized cloud applications gain popularity and replace VM-based architecture, it is important to understand how Kubernetes handles YoYo attacks. In this paper, we analyze the resilience of Kubernetes auto-scaling against YoYo attacks. We model the underlying auto-scaling mechanism and show that it is still very vulnerable to YoYo attacks, because VMs are still involve in this mechanism. Given that, we propose a novel approach to detect a YoYo attack on a Kubernetes cluster based on machine learning methodology.  We demonstrate the YoYo attack and its mitigation on a Google Kubernetes Engine cluster.}



\ignore{
Auto-scaling mechanism is an important line of defense against DDoS in the cloud \cite{amazon}.  The auto-scaling mechanism translates the DDoS attacks into  Economic Denial of Sustainability attack (EDoS), where the victim suffers from economic damage incurred by paying  the extra resources required to process the bogus traffic of the attack.
Recent work presents a new kind of attack, the Yo-Yo attack \cite{8057010} that causes significant performance degradation in addition to economic damage. In the Yo-Yo attack, the attacker sends periodic bursts of overload, thus causing the auto-scaling mechanism to oscillate between scale-up and scale-down phases. The attack \cite{8057010} was demonstrated using  VM auto-scaling in AWS. In this scenario, during the scale-up time, that can takes several minutes, the victim suffers from substantial performance degradation. 
 
 \emph {In this research we analyze the resilience of  Kubernetes auto-scaling  against Yo-Yo attacks.}    Kubernetes is a commonly used open source container orchestration platform. It is interesting to analyze the resilience of Kubernetes to  YoYo attack since the scale-up time  of containers is much lower than VM. \ignore{ We modeled the Yo-Yo attack under two policies of Kubernetes, HPA (i.e Horizontal Pod Auto-scaler) and Cluster Autoscaling. We  evaluated the Performance and Economic Damage. Finally we evaluate models that can accurately detect Yo-Yo attack.}
 
 
\ignore{ by reducing the cost of scaling using containers. however the economic cost could be significant unless customer purchase insurance plans from Cloud vendors by purchasing costly premium services or Reblaze\texttrademark DDos protection.}
We modeled the Yo-Yo attack under two policies of Kubernetes, HPA (i.e Horizontal Pod Auto-scaler) and Cluster Autoscaling. We evaluated the Performance and Economic Damage and investigate the vulnerability of auto-scaling as a defense method under the new conditions including setting minimum and maximum compute power to scale 
\ignore {including assigning  predictive mechanism in the cloud provider.} We analyzed the economic impact that could mislead the auto-scale prediction methods causing them to an unexpected behavior and fail on resource estimation.
}
